Solving the "many variables" problem in MICE with principal component regression

Multiple Imputation (MI) is one of the most popular approaches to addressing missing values in questionnaires and surveys. MI with multivariate imputation by chained equations (MICE) allows flexible imputation of many types of data. In MICE, for each variable under imputation, the imputer needs to specify which variables should act as predictors in the imputation model. The selection of these predictors is a difficult, but fundamental, step in the MI procedure, especially when there are many variables in a data set. In this project, we explore the use of principal component regression (PCR) as a univariate imputation method in the MICE algorithm to automatically address the "many variables" problem that arises when imputing large social science data. We compare different implementations of PCR-based MICE with a correlation-thresholding strategy by means of a Monte Carlo simulation study and a case study. We find the use of PCR on a variable-by-variable basis to perform best and that it can perform closely to expertly designed imputation procedures.

==> section_01.tex <==
% Project:  paper-mipcr-compare
% Topic:    Introduction
% Author:   Edoardo Costantini
% Created:  2021-12-17
% Modified: 2022-06-30

\section{Introduction}\label{sec:introduction}

Missing values are a problem afflicting virtually all data sets in the social and behavioral sciences.
Multiple Imputation (MI) is one of the most popular approaches to address the issue of non-response.
Although MI can treat essentially any missing data problem, it was originally designed to impute large surveys, especially when those surveys are used to create publicly released data that many researchers will analyze independently \citep{rubin:1996}.
In this context, MI was envisioned as being especially useful when the data collector (and imputer) is distinguished from the ultimate user (or analyst).

The imputer's main task is to define an imputation model that supports analyses from many users.
A well-designed imputation model should include all the predictors of missingness present in the data, and it should incorporate all the features of the substantive analysis models that will be used by the data analysts.
If important predictors of missingness are left out of the imputation model, the missing at random (MAR) assumption is violated~\citep[p. 339]{collinsEtAl:2001}.
If some features of the substantive analysis model of interest do not appear in the imputation model, the two models are said to be uncongenial, a situation that can invalidate the inferential conclusions obtained after imputation (\citealp{meng:1994};~\citealp[p. 218]{littleRubin:2002}.)

To decide which predictors to include in the imputation model, a commonly recommended strategy is to include as many predictors as possible \citep[i.e., the inclusive strategy, ][]{collinsEtAl:2001}.
However, the scale of modern social surveys and data collection endeavors complicates the task of selecting these predictors.
Cross-sectional social surveys (e.g., World values survey \citealp{WVS:2020}; European values study, \citealp{EVS:2017}) commonly measure hundreds of variables, and including all of these variables in the imputation model can lead to prohibitively long imputation times and convergence failures \citep[p. 259]{vanBuuren:2018}.
Social and behavioral scientists also frequently work with longitudinal surveys and panel studies (e.g., Panel Study of Income Dynamics, \citealp{mcgonagleEtAl:2012}; LISS Panel, \citealp{LISS:2018}), which can lead to data sets with many more columns than rows.
This high-dimensionality can result in singularity issues \citep[p. 46]{hastieEtAl:2009} when estimating the imputation models.
The imputer needs to address this ``many variables'' problem by thoroughly scanning all the available variables to decide which of them should be used in the imputation models.
In this article, we explore the use of principal component regression to automate the definition of the imputation model by replacing a large number of possible predictors with a small subset of principal components (PCs).

\subsection{MICE and the ``many variables'' problem}

In social science research, multivariate imputation by chained equation~\citep[MICE][]{mice} has been implemented in all major statistical software (e.g., \citealp{statacorp:2013}; \citealp{IBM:2020}; \citealp{mice}) and is arguably the most popular way to implement MI\@.
MICE, also known as fully conditional specification, is an iterative algorithm that obtains imputations from the multivariate distribution of the missing data by sampling from a set of univariate conditional densities.
This algorithm requires the definition of a conditionally specified univariate imputation model for each variable under imputation.
At every iteration, each univariate imputation model is used to obtain replacement values for the missing data points.
When convergence is reached, any sample from the univariate imputation models' predictions represents a sample from the target multivariate data distribution.
These samples are used to define multiple versions of the original data, with different plausible values used to replace the original missing data.
Any analysis model of scientific interest can then be estimated on each of the multiply imputed datasets.
The estimates of the parameters of interest in the analysis model are then pooled following Rubin's rules~\citep[p. 76]{rubin:1987}.

The definition of the univariate imputation models is a fundamental step for the good performance of the MICE procedure.
For each variable under imputation, the imputer needs to define a univariate imputation model.
The task involves two decisions:
\begin{enumerate}
    \item Selection of the model form;
    \item Selection of the model predictors.
\end{enumerate}

The first point is usually guided simply by the measurement level of the variables under imputation.
For example, continuous variables can be imputed using a linear regression model, while binary variables can be imputed using logistic regression.
The second point consists of choosing the variables to be included as predictors in the imputation model.
In general, it is advisable to adopt an inclusive strategy~\citep{collinsEtAl:2001}, meaning including as many predictors as possible in the univariate imputation models.
Using as much information as possible from the data leads to multiple imputations that have minimal bias and maximal efficiency~\citep{meng:1994, collinsEtAl:2001}.
Furthermore, including more predictors in the univariate imputation models makes the MAR assumption more plausible~\citep[p. 339]{collinsEtAl:2001}.
Finally, if the imputation model omits variables that are part of the analysis model fitted to the data, the parameter estimates might be biased \citep[p. 229]{enders:2010} and estimated confidence intervals might be too wide \citep[p. 218]{littleRubin:2002}.
As a result, including more predictors in the imputation models increases the range of analysis models that can be estimated with a given set of imputations~\citep{meng:1994}.

When a data set consists of only a few variables (i.e., tens of variables), it is feasible to include all of these variables in all the univariate imputation models.
However, standard imputation methods face computational limitations in the presence of a large number of predictors (i.e., hundreds).
For example, MICE using Bayesian imputation under the normal linear model~\citep[p. 68]{vanBuuren:2018} requires the number of predictors ($p$) in the univariate imputation model to be smaller than the number of observed cases ($n$) to avoid computational problems with the system of equations~\citep[p. 203]{jamesEtAl:2013}.
Even when the number of predictors is smaller than the number of observations, the inclusion of many predictors in the imputation models can increase the chances of collinearity issues~\citep[pp. 167--170]{vanBuuren:2018} and biased analysis model parameter estimates~\citep{hardtRainer:2012}.

The type of data social and behavioral scientists work with today often contains many variables.
For example, a single wave of the World Values Survey \citep{WVS:2020} contains more than 300 variables, and a single wave of the European Values Study \citep{EVS:2017} contains around 250 variables.
Running a MICE algorithm on this type of data, without selecting a subset of variables to use as predictors in the univariate imputation models, requires the algorithm to estimate regression models with hundreds of predictors for each variable under imputation.
With such a specification, the algorithm will be extremely slow, and the imputations will be poor.
However, the selection of a smaller subset of predictors for each univariate imputation model can be a daunting task.
Choosing which predictors should be included in the univariate imputation models that constitute a run of the MICE algorithm entails a degree of subjectivity, requiring experience to achieve satisfactory results.

\citet[pp. 270--271]{vanBuuren:2018} provides a summary of different strategies an expert imputer can take when designing imputation for social science data sets with many variables.
The imputer can:
\begin{enumerate}
    \item Remove constants and collinear variables.                      \label{item:colli}
        Collinear predictors will lead to unstable imputation model parameter estimates.
        Using one of a set of collinear predictors reduces the size of the predictor space for imputation models without losing any important information.
    \item Evaluate statistics describing the connection between variables in the data. \label{item:iopat}
        For example, one can compute the proportion of usable cases for imputing a variable based on another \citep[i.e., inbound statistic][p. 108]{vanBuuren:2018}.
        The more cases that are usable, the more \textit{connected} the two variables are.
        The influx-outflux coefficients \citep[pp. 109--111]{vanBuuren:2018} provide overall measures of how each variable \textit{connects} to the rest of the data.
        In general, variables with high influx and outflux are preferred as predictors in an imputation model.
    \item Apply a correlation-thresholding strategy.                 \label{item:quickpred}
        Only variables that are associated with the variables under imputation can be effective predictors in the imputation models.
        As a result, a good strategy to select a small number of important predictors is to include only variables that correlate with the ones under imputation more strongly than a chosen threshold.
        However, while choosing a low threshold might lead to selecting too many variables, choosing a high threshold might lead to excluding important predictors.
\end{enumerate}

These strategies are not guaranteed to avoid over-parametrization of the univariate imputation models, and often more strategies are needed.
The nature of social science data offers a few other opportunities to reduce the dimensionality of the imputation models.
For example, with longitudinal data sets, the imputer might decide to use only the first measurement of the same construct when imputing other variables, or she may use the total score in place of the many items constituting a scale.
Additionally, an imputer can use high-dimensional prediction methods as univariate imputation models. 
Shrinkage methods, non-parametric models, and dimension reduction can be used in MICE to reduce the complexity of the predictors' selection step.
\citet{zhaoLong:2016} and \citet{dengEtAl:2016} proposed the use of lasso variable selection \citep{tibshirani:1996} within MICE, a shrinkage technique that provides a data-driven selection of important predictors for each imputation model.
Decision trees allow the inclusion of more predictors than traditional parametric imputation methods~\citep{burgetteReiter:2010, dooveEtAl:2014, shahEtAl:2014}, and they have been integrated in popular packages (e.g., \cite{mice}) for the software environment R \citep{R:2020}.
\citet{howardEtAl:2015} proposed the use of dimension reduction of auxiliary variables through principal component analysis~\citep[PCA;][pp. 1--6]{jolliffe:2002}.
By extracting principal components (PCs) from the set of possible auxiliary variables, this method summarizes the information contained in the large set of predictors with just a few variables.
These PCs can then be used as predictors in a standard, low-dimensional application of MICE\@.

The approaches described above have the potential to automatically address the issues of having too many variables available as possible imputation model predictors.
By default, high-dimensional prediction models avoid collinearity issues and hence stabilize imputation model estimation.
Furthermore, high-dimensional methods usually offer some form of variable selection or dimensionality reduction that can reduce the burden of making predictor choices.
Finally, by allowing the inclusion of more predictors in the imputation model, high-dimensional prediction models may get as close as possible to imputation under MAR, given the available data.

An expert setup of the MICE algorithm may lead to better imputations than using automatic, data-driven, approaches (though, as we illustrate in Section \ref{sec:case-study}, this need not always be the case).
However, expert knowledge is not always available for every project that could benefit from imputation.
Furthermore, high-dimensional prediction models do not need to be the sole solution to the ``many variables'' imputation problem.
They can always be combined with expert knowledge to further improve the quality of imputation.

\cite{costantiniEtAl:2022} studied a wide range of high-dimensional MI approaches and found that the use of PCA to reduce the dimensionality of the imputation models consistently led to small estimation bias and close-to-nominal confidence interval coverage of the true analysis model parameters values compared with other methods considered.
However, that study was limited to a single implementation of PCA\@.
In this paper, we compared three approaches to using PCA as a dimensionality reduction technique for MICE\@.
Two approaches have been previously described in the literature, and we propose a novel third method here.

\subsection{Principal component analysis for MICE}\label{subsec:principal-component-analysis-for-mice}

PCA is a dimensionality reduction technique by which a set of variables is summarized with a smaller number of PCs that collectively explain the largest possible proportion of the original data's variance, given the number of PCs.
PCA can be used in conjunction with many statistical techniques, and its use in regression analysis has been extensive \citep[e.g.,][]{deJongKiers:1992, rosipalEtAl:2001, reissTodd:2007, parkEtAl:2021}.
In particular, one of the best-known uses of PCA in multiple regression is principal component regression~\citep[PCR;][pp. 168--173]{jolliffe:2002}, where PCs act as predictors in a multiple regression model.

Standard implementations of the MICE algorithm cycle through many univariate imputation models that can be replaced by PCR\@.
We refer to this use of PCA in conjunction with MICE as MI-PCR\@.
This is a broad approach that can be implemented in different ways.
PCs may be estimated before using MICE to create a small set of covariates that are then used in a subsequent run of MICE as imputation model predictors.
Alternatively, PCA may be used within every iteration of MICE, by estimating new PCs at every iteration based on the most recent imputations.
In this report, we investigate how different uses of PCA impact imputation quality.

We also explore how the number of components used influences imputation.
Based on their analysis of data with a simple unidimensional latent structure, \citet{howardEtAl:2015} proposed to either select the first PC, or enough PCs to explain 40\% of the variance in the possible predictors.
However, medical and social science data are characterized by complex latent structures that might not be well summarized by a single component.
Therefore, studying the impact of this decision is another key interest of the present study.
Finally, we study different characteristics of the data that can make MI-PCR more or less effective for imputation.
In particular, the measurement level and the strength of association between the variables on which PCs are computed might impact the performance of MI-PCR\@.

In this manuscript, we present the results of a Monte Carlo simulation study where we explored the impact of such aspects on the imputation performance of MI-PCR\@.
Imputation performance is assessed based on the estimation bias, confidence interval width, and confidence interval coverage (see Section \ref{subsubsec:analysis-and-outcome-measures} for details).
We also compare the different implementations of MI-PCR to impute the Fireworks Disaster data---a real clinical psychology data set---and a popular case study for high-dimensional imputation problems~\citep[p. 313]{vanBuuren:2018}.
In what follows, we describe how PCA can be used within the MICE algorithm (Section \ref{sec:mi-pcr-mice-using-pcr}).
We then discuss the simulation study and the case study in Sections \ref{sec:simulation-study} and \ref{sec:case-study}, respectively.
In Section \ref{sec:limitations}, we discuss limitations and future research directions, and we discuss our conclusions in Section \ref{sec:conclusions}.


==> section_02.tex <==
% Project:  paper-mipcr-compare
% Topic:    Description of imputation methods
% Author:   Edoardo Costantini
% Created:  2021-12-17
% Modified: 2022-06-08

\section{MI-PCR: MICE using PCR}\label{sec:mi-pcr-mice-using-pcr}

Here we briefly describe the MICE algorithm, PCA, and how PCA can be used in conjunction with MICE\@.
We use the following notation.
Scalars are denoted by lowercase letters in light typeface (non-bold).
Vectors and matrices are denoted by bold lowercase and bold uppercase letters, respectively.
We use the superscripts $obs$ and $mis$ to refer to the observed and missing elements in a vector.
For a given data set, we refer to the variables that are part of the researcher's substantive model of scientific interest (e.g., the linear regression used to answer a research question) as \text{analysis variables}.
We refer to all other variables as \text{potential auxiliary variables} for the imputation models.
We use the subscripts $am$ and $ax$ to refer to variables that are part of either the analysis model or the set of potential auxiliary variables, respectively.

\subsection{Multivariate imputation by chained equations}\label{subsec:multiple-imputation-chained-equations}

Consider an $n \times p$ data set $\bm{X}$.
Its columns, $\bm{x}_1, \dots, \bm{x}_p$, represent variables recorded by a data collector.
Assume the first $t$ columns of $\bm{X}$ have missing values.
For each partially observed $\bm{x}_j$, with $j = 1, \dots, t$, the imputer defines a univariate imputation model:
%
\begin{equation} \label{eq:uim}
    f(\bm{x}_j|\bm{X}_{-j}, \bm{\theta}_j),
\end{equation}
%
where $\bm{X}_{-j}$ is the collection of variables in $\bm{X}$ excluding $\bm{x}_{j}$, and $\bm{\theta}_j$ is a vector of imputation model parameters.
Model \ref{eq:uim} is usually a generalized linear model chosen according to the measurement level of $\bm{x}_j$.
The MICE algorithm starts with replacing the missing values in each $\bm{x}_j$ with initial guesses.
Then, at every iteration, each variable is imputed by its univariate imputation model.
First, the imputation model parameters are drawn from their fully conditional posterior distribution, and then imputations are drawn from the posterior predictive distribution of $\bm{x}_j$.

For the $j$th variable under imputation at iteration $k$, the algorithm draws from the following distributions:
%
\begin{align}
    \bm{\theta}_j^{(k)} &\sim f(\bm{\theta}_j)f(\bm{x}_j^{obs}|\bm{X}_{-j}^{(k)}, \bm{\theta}_j) \label{eq:post_dist}, \\
    \bm{x}_j^{mis(k)} &\sim f(\bm{x}_j^{mis}|\bm{X}_{-j}^{(k)}, \bm{\theta}_j^{(k)})                \label{eq:pred_dist}
\end{align}
%
Equation~\ref{eq:post_dist} is the fully conditional posterior distribution defined as the product of $f(\bm{\theta}_j)$, a prior distribution for $\bm{\theta}_j$, and $f(\bm{x}_j^{obs}|\bm{X}_{-j}^{(k)}, \bm{\theta}_j)$, the likelihood of observing $\bm{x}_j^{obs}$ under the imputation model for $\bm{x}_j$.
Equation~\ref{eq:pred_dist} is the posterior predictive distribution from which updates of the imputations are drawn.
In both equations, $\bm{X}_{-j}^{(k)}$ is $(\bm{x}_1^{(k)}, \dots, \bm{x}_{j-1}^{(k)}, \bm{x}_{j+1}^{(k-1)}, \dots, \bm{x}_{p}^{(k-1)})$, meaning that at all times the most recently imputed values of all variables are used to impute other variables.

After cycling through all $t$ variables under imputation, the algorithm moves to the next iteration.
After a sufficient number of iterations, the algorithm converges and the imputations are assumed to be samples from the target multivariate distribution.
With this process, one can generate as many imputed data sets as desired.
Finally, the analysis model is estimated on each imputed data set, and the parameter estimates are pooled appropriately using Rubin's rules \citep{rubin:1987}.

\subsection{Principal component analysis}\label{subsec:principal-component-analysis}
PCA finds a low-dimensional representation of the large set of variables contained in $\bm{X}$ with minimal loss of information.
We refer to this low-dimensional representation as the $n \times q$ matrix $\bm{Z}$, where $q < p$.
The columns of $\bm{Z}$ are called the principal components (PCs) of $\bm{X}$.
The first PC of $\bm{X}$\footnote{We follow the common practice of assuming that the columns of $\bm{X}$ are mean-centered and scaled to have a variance of 1.} is the linear combination of the columns of $\bm{X}$ with the largest variance:
%
\begin{equation} \label{eq:z1}
    \bm{z}_1 = \bm{x}_1 \lambda_{11} + \bm{x}_2 \lambda_{12} + \dots + \bm{x}_p \lambda_{1p} = \bm{X} \bm{\lambda}_1,
\end{equation}
%
with $\bm{\lambda}_1$ being the $p \times 1$ vector of weights $\lambda_{11}, \dots, \lambda_{1p}$.
The second principal component ($\bm{z}_2$) is defined by finding the vector of weights $\bm{\lambda}_2$ giving the linear combination of $\bm{x}_1, \dots, \bm{x}_p$ with maximal variance out of all the linear combinations that are uncorrelated with $\bm{z}_1$.
Every subsequent column of $\bm{Z}$ can be understood in the same way: for example, $\bm{z}_3$ is the linear combinations of $\bm{x}_1, \dots, \bm{x}_p$ that has maximal variance out of all the linear combinations that are uncorrelated with $\bm{z}_1$ and $\bm{z}_2$.
As a result, all PCs are uncorrelated by definition and every subsequent PC has a lower variance than the preceding one.
We can write the relationship between all the PCs and $\bm{X}$ in matrix notation:
%
\begin{equation} \label{eq:PCAmatnot}
    \bm{Z} = \bm{X} \bm{\Lambda},
\end{equation}
%
where $\bm{\Lambda}$ is a $p \times q$ matrix of weights, with columns $\bm{\lambda}_1, \dots, \bm{\lambda}_q$.
Equation~\ref{eq:PCAmatnot} also allows us to understand PCA as the process of projecting the original data from a $p$-dimensional space to a $q$-dimensional space.
The weight vectors $\bm{\lambda}_1, \dots, \bm{\lambda}_q$ define the directions in which the $n$ observations of $\bm{x}_1, \dots, \bm{x}_p$ are projected.
The projected values are the principal component scores $\bm{Z}$.

\subsection{Principal component regression}\label{subsec:principal-component-regression}

PCR replaces the $p$ predictors of a regression model with $q$ PCs extracted from those predictors.
Given the data $\bm{X}$, consider a standard regression model where the $j$th variable is regressed on the other columns in the data:
%
\begin{equation} \label{eq:lm}
    \bm{x}_j = \bm{X}_{-j}\bm{\beta} + \epsilon,
\end{equation}
%
where $\bm{x}_j$ is a $n \times 1$ vector of dependent variable scores, $\bm{\beta}$ is a $(p - 1) \times 1$ vector of $p - 1$ regression coefficients, and $\epsilon$ is a $n \times 1$ vector of independent normally distributed errors.
With PCR we use the PCs of $\bm{X}_{-j}$ in place of $\bm{X}_{-j}$ in the regression model so that Equation~\ref{eq:lm} can be rewritten as:
%
\begin{equation} \label{eq:PCR}
    \bm{x}_j = \bm{Z}\bm{\gamma} + \epsilon,
\end{equation}
%
where $\bm{\gamma}$ is a $q \times 1$ vector of regression coefficients.
The lower dimensionality of $\bm{Z}$ compared to $\bm{X}_{-j}$, and the independence of its columns, allow Equation~\ref{eq:PCR} to address the computational limitations of Equation~\ref{eq:lm} in the presence of many predictors.

\subsection{MI-PCR}\label{subsec:mi-pcr}
Standard MICE formulations are based on univariate imputation models that suffer from the same computational limitations as we discussed for multiple regression.
In general, the idea of MI-PCR is to use Equation~\ref{eq:PCR} as the univariate imputation model for every variable under imputation.
By doing so, we aim to address the ``many variables'' problem by summarising the imputation models' predictors with just a few PCs.
However, this idea can be implemented in many ways.
PCA can be used at different stages of the MICE algorithm, and different sets of variables can be summarised by the PCs.
In the following sections, we describe the three implementations evaluated in this study.

\subsubsection{MICE with PCA on auxiliary variables}

The most straightforward way to use PCA within MICE is to compute a single set of PCs based only on the potential auxiliary variables.
In general, potential auxiliary variables include predictors of missingness, variables related to the ones under imputation, and variables that are useless for imputation.
To reduce the dimensionality of imputation models, an expert imputer would usually examine these variables to locate and exclude members of the last group from the imputation models.
PCA can be used as an alternative, data-driven pre-processing step to project all the possible auxiliary variables onto a lower-dimensional space and bypass the need to select which variables to use as predictors in the imputation models.
We refer to this approach as MICE with PCA on the auxiliary variables (MI-PCR-AUX).

In MI-PCR-AUX, the univariate imputation models use as predictors the raw version of any variable that is part of the analysis model, and the principal components summarising the potential auxiliary variables.
We can write the univariate imputation model as:
%
\begin{equation} \label{eq:MIPCRaux}
    f(\bm{x}_j|\bm{X}_{am, -j}, \bm{Z}_{ax}, \bm{\theta}_j),
\end{equation}
%
where $\bm{X}_{am, -j}$ is the set of analysis model variables except the one under imputation, and $\bm{Z}_{ax}$ is the set of PCs estimated from the set of possible auxiliary variables $\bm{X}_{ax}$.
This use of PCA was proposed by~\cite{howardEtAl:2015}.

The strength of MI-PCR-AUX is using the raw analysis model variables (not filtered via the PCA) while including as much auxiliary information as possible (filtered via the PCA).
However, MI-PCR-AUX requires knowledge of the analysis model before imputation, and the possible presence of missing values in the potential auxiliary variables needs to be addressed.
\cite{howardEtAl:2015} suggested using single imputation to create a complete set of potential auxiliary variables, but all the obstacles to defining the univariate imputation models previously discussed would then need to be faced for this single imputation procedure.

\subsubsection{MICE with PCA on all variables}

One way to relax the requirements of knowing the analysis model before running the imputation procedure is to extract PCs from all available variables---including the ones under imputation---and then use only these PCs as predictors in the imputation models.
This approach is implemented in the R package \textit{PcAux}~\citep{PcAux}.
We refer to it as MI-PCR-ALL\@.
The univariate imputation model for this approach can be written as:
%
\begin{equation} \label{eq:MIPCRall}
    f(\bm{x}_j|\bm{Z}, \bm{\theta}_j),
\end{equation}
%
where $\bm{Z}$ is the set of PCs estimated on $\bm{X}$.
Ideally, MI-PCR-ALL supports a wide range of analysis models, as the information on every available variable is summarised by the PCA procedure and included in all the imputation models.
In theory, the imputer could even augment $\bm{X}$ before extracting the PCs with every desired interaction and polynomial term that might be present in an analysis model.

PCA cannot be performed in the presence of missing values.
As we are performing PCA on all the variables in $\bm{X}$---even the ones targeted by imputation---we must first (temporarily) treat the missing data to allow the PC extraction.
Our implementation of MI-PCA-ALL begins by filling in the missing values with a single imputation run and subsequently extracting PCs from this completed data set.
It is important to note that these imputations will not be used for statistical inference.
Therefore, as long as the imputations are well-constructed and are consistent with the distribution of the original variables, the inference based on MI-PCR-ALL should not be negatively impacted.
Nevertheless, the performance of this method relies on the quality of this first single imputation.

In MI-PCA-ALL, the PCs are the only predictors used in the univariate imputation models and do not have missing values.
Therefore, a single iteration of the MICE algorithm is sufficient.
Computationally, this is an advantage as there is no need to perform any burn-in iterations.

\subsubsection{MI with PCA on a variable-by-variable basis}

The most flexible way to incorporate PCA into MICE is to extract PCs at every iteration.
When imputing $\bm{x}_j$ at the $k$th iteration, PCs can be estimated from $\bm{X}^{(k)}_{-j}$ and used as predictors in the univariate imputation model.
Each univariate imputation model can then be defined as:
%
\begin{equation} \label{eq:MIPCR}
    f(\bm{x}_j|\bm{Z}_{-j}, \bm{\theta}_j),
\end{equation}
%
where $\bm{Z}_{-j}$ is the matrix storing the PC scores estimated on $\bm{X}^{(k)}_{-j}$.
We refer to this approach as MI-PCR-VBV because of the variable-by-variable use of PCA\@.

As with MI-PCA-ALL, MI-PCR-VBV does not require knowledge of the analysis model prior to imputation and it can support a wide range of analysis models.
Moreover, by extracting PCs at every iteration from variables with the most recently imputed values, MI-PCR-VBV addresses missing values in one step, without requiring a pre-processing single imputation procedure.
The disadvantage of MI-PCR-VBV is in the higher computational intensity relative to both MI-PCR-AUX and MI-PCR-ALL\@.
Performing PCA on large social surveys involves demanding matrix operations.
MI-PCR-VBV requires repeating these intensive manipulations for every variable under imputation and for every iteration of the MICE algorithm.


==> section_03.tex <==
% Project:  paper-mipcr-compare
% Topic:    Methods for the paper
% Author:   Edoardo Costantini
% Created:  2021-12-17
% Modified: 2022-06-10

\section{Simulation study}\label{sec:simulation-study}

We investigated the relative performance of the methods described above with a Monte Carlo simulation study.
In particular, we were interested in assessing the estimation bias, confidence interval width, and confidence interval coverage of some analysis model parameters obtained after imputation.
The purpose of this study was to evaluate these statistical properties of MI-PCR in several settings that differed in the proportion of noise variables present in the data, the measurement level of the variables, and the number of PCs used in the imputation models.

When defining the univariate imputation model, an expert imputer would usually exclude all variables that are weakly associated with the ones under imputation.
We refer to these weak predictors of the imputation targets as noise variables.
When using MI-PCR, noise variables will contribute to the construction of the PCs as much as the important predictors of the variables under imputation.
Consequently, PCs extracted from data that contain a large proportion of noise variables may be more weakly associated with the variables under imputation.
We expect that the presence of a larger proportion of noise variables will negatively impact the performance of MI-PCR\@ (i.e., larger bias, lower efficiency, larger deviation from nominal coverage).
Additionally, in real survey applications, theoretical constructs of interest are often measured with discrete items such as Likert scales.
The number of categories with which information is recorded in a variable can have a strong impact on how well $\bm{Z}$ represents $\bm{X}$.
On the one hand, MI-PCR might perform worse when fewer categories are used to record the data.
On the other hand, PCA finds continuous components that might adequately represent the underlying latent structure of discrete items.
Finally, each of the implementations of MI-PCR described above can be used with different numbers of PCs.
\cite{howardEtAl:2015} suggested that using the first PC may be sufficient.
However, they used a set of strongly associated potential auxiliary variables measuring a single latent factor.
When the underlying correlation structure is more complex (i.e., more than one latent factor, different correlation levels) using only the first PC is likely to result in a poor representation of the data and poor imputation performance.
In what follows we outline the simulation study procedure, discuss the experimental factors in detail, and report the results.

\subsection{Method}

The simulation study procedure involved four steps:
\begin{enumerate}
    \item Data generation: We generated 500 data sets ($S = 500$) from a confirmatory factor analysis model, following the procedure described in Section \ref{subsubsec:data-generation}.
    \item Missing data imposition: We imposed missing values on four target items in each generated data set, following the procedure described in Section \ref{subsubsec:missing-data-imposition}.
    \item Imputation: We generated $d$ multiply imputed data tables for each generated data set using each of the different imputation methods, as described in Section \ref{subsubsec:imputation-procedures}.
    \item Analysis: We estimated the means, variances, covariances, and correlations of the four items with missing values on the $d$ differently imputed data tables, and we pooled the estimates according to Rubin's rules \citep[p. 76]{rubin:1986}.
    We then assessed the performance of each imputation method by computing the bias, confidence interval width, and confidence interval coverage of the true parameter values as described in Section \ref{subsubsec:analysis-and-outcome-measures}.
\end{enumerate}
\subsubsection{Data generation}\label{subsubsec:data-generation}

For each replication, we generated a $500 \times 58$ matrix of fully observed data $\bm{X}$.
We fixed the sample size to 500 observations to generate data sets that would have statistical properties similar to large social science data sets without needlessly increasing the computational demands of the simulation study.
Each data set was generated based on the following confirmatory factor analysis model:
%
\begin{equation} \label{eq:CFAmod}
    \bm{X} = \bm{F}\bm{\Lambda}' + \bm{E},
\end{equation}
%
where $\bm{F}$ is a $500 \times 7$ matrix of latent variables scores, $\bm{\Lambda}$ is a $56 \times 7$ matrix of factor loadings, $\bm{\Lambda}'$ is its transpose, and $\bm{E}$ is a $500 \times 56$ matrix of measurement errors.

The factor loading matrix $\bm{\Lambda}$ described a simple measurement structure~\citep[p. 234]{bollen:1989} where every item loads on a single factor.
The factor loadings were set to the fixed value of $\lambda = 0.85$.
Standardized factor loadings in social science data sets are often in the range of $(0.6, 0.85)$.
We generated data with relatively high factor loadings because we wanted to mitigate the impact of measurement error on our findings without resorting to implausibly precise data.
We sampled the latent scores for seven factors from a multivariate normal distribution with mean $\bm{0}$ and covariance matrix $\bm{\Psi}$:
%
\begin{equation} \label{eq:Psi}
\bm{\Psi} =
    \begin{bmatrix}
    1           & \psi_{12} & \dots & \psi_{17} \\
    \psi_{21}   & 1         & \dots & \psi_{27} \\
    \dots       & \dots     & \dots & \dots \\
    \psi_{71}   & \psi_{72} & \dots & 1 \\
    \end{bmatrix}.
\end{equation}
%
The matrix of measurement errors $\bm{E}$ was sampled from a multivariate normal distribution with mean vector $\bm{0}$ and covariance matrix $\bm{\Theta}$.
The off-diagonal elements of $\bm{\Theta}$ were set to 0 to reflect uncorrelated errors, while the diagonal elements were specified as $1 - \lambda^2$ to give the simulated items unit variances.
After sampling, data were rescaled to have approximately a mean of 5 and a variance of 6.5, which are common values for Likert items in social surveys measured on a 10-point scale.

Each data matrix generated with the procedure described above was partitioned into three sub-matrices:
%
\begin{equation}
    \bm{X} = (\bm{T}, \bm{M}, \bm{A}) \label{eq:Xpart}
\end{equation}
%
where:
\begin{itemize}
    \item $\bm{T}$ is an $n \times 4$ matrix consisting of the first four indicators ($\bm{x}_1, \dots, \bm{x}_4$) of the first latent variable $\bm{f}_1$. 
    We imposed missing data on these items as described in Section \ref{subsubsec:missing-data-imposition}.
    \item $\bm{M}$ was an $n \times 4$ matrix consisting of the other four items ($\bm{x}_5, \dots, \bm{x}_8$) measuring the first latent variable.
    These items were used to define the probability of nonresponse for the items in $\bm{T}$ as described in Section \ref{subsubsec:missing-data-imposition}.
    \item $\bm{A}$ was an $n \times 48$ matrix consisting of 48 items measuring the the remaining six latent variables $\bm{f}_2, \dots, \bm{f}_7$.
\end{itemize}

In generating the data, we varied two design factors: the number of categories for the coarsened potential auxiliary variables ($nk = \infty, 7, 5, 3, 2$), and the proportion of noise variables ($pn$ = 0, 0.33, 0.67, 1).
We crossed these factors in a $5(nk) \times 4(pn)$ factorial design.
We considered the variables in $\bm{M}$ and $\bm{A}$ as the pool of potential auxiliary variables and we discretized them according to the $nk$ factor to study the impact of data coarseness on the performance of the imputation methods.
The $nk = \infty$ level represents the uncoarsened, continuous variables.
We used the $pn$ factor to define the proportion of noise variables in $\bm{A}$.
That is, the proportion of items in $\bm{A}$ that are uncorrelated with the ones in $\bm{T}$.
We controlled this factor at the latent variable level through the values of $\psi_{jk}$, the latent correlation in Equation~\ref{eq:Psi}.
When $pn = 0.33$, two out of the six latent variables indicated by the items in $\bm{A}$ had a low correlation ($0.1$) with $\bm{f}_1$, and the remaining four had a high correlation ($0.7$) with $\bm{f}_1$.
As a result, one-third of the items in $\bm{A}$ were also lowly correlated with the items in $\bm{T}$ and $\bm{M}$.
When $pn = 0$, all latent variables were correlated at 0.7, so every variable in $\bm{A}$ correlated highly with the ones in $\bm{T}$ and $\bm{M}$.
When $pn = 1$, all latent variables were correlated at 0.1, so all variables in $\bm{A}$ were trivially correlated with the ones in $\bm{T}$ and $\bm{M}$.

\subsubsection{Missing data imposition} \label{subsubsec:missing-data-imposition}

We imposed missing values in $\bm{T}$ by first generating an indicator of missingness ($\delta$) for each column of $\bm{T}$.
When the indicator took value 0, we left the original sampled value; when the indicator took value 1, we replaced the sampled value with a missing value.
The indicator was produced by sampling from Bernoulli distributions with probabilities defined based on the following logit model:
%
	\begin{equation} \label{eq:logit}
		logit(\delta = 1) = \beta_0 + \bm{M}\bm{\beta},
	\end{equation}
%
where $\beta_0$ is an intercept parameter, and $\bm{\beta}$ is a vector of slope parameters, so that the probability of nonresponse is a linear combination of the predictors in $\bm{M}$.
Because only the variables in $\bm{M}$ were used to predict missingness in $\bm{A}$, the probability of nonresponse for a variable never depended on the variable itself.
All slopes in $\bm{\beta}$ were fixed to 1, while the value of $\beta_0$ was chosen with an optimization algorithm that minimized the difference between the actual and desired proportion of missing values\footnote{
The pseudo R-squared for the logistic regression of the missing value indicator on the predictors of missingness was approximately 14\%.
The AUC for the logistic regression was approximately 0.74.
}.
The proportion of missing values per variable was set to 0.3.
Although this value is high for social science data, it is not exceptional, and imposing more missing data granted a stronger distinction between the imputation methods' performances, compared to lower values we could have chosen.

Missingness was imposed using $\bm{M}$ in its original continuous form, even in those conditions where the possible auxiliary variables were coarsened (i.e., $nk \neq \infty$).
We made this decision to maintain the strength of the MAR mechanism as consistently as possible across conditions.
Using the coarsened versions of $\bm{M}$ to impose missing values would have generated a weaker MAR relation (closer to missing completely at random, MCAR) for conditions with lower numbers of categories.
Doing so would have led, by design, to slightly better performance for every method for data discretized to fewer categories.
At the same time, the solution we adopted is also imperfect.
For a lower number of categories, the data available to be used as predictors in the imputation models were worse representations of the actual MAR predictors.
As a result, one might argue that, for the conditions with fewer categories, imputation was closer to a missing not at random (MNAR) situation rather than MAR.
When designing the study we reasoned that making imputation more difficult (closer to MNAR) rather than easier (closer to MCAR) would be more informative.

\subsubsection{Imputation procedures}\label{subsubsec:imputation-procedures}

After generating the data and imposing missing values, every variable in $\bm{T}$ was imputed with the three versions of MI-PCR described above:
 \begin{itemize}
    \item MI-PCR-AUX\@.
            The PCs used in the univariate imputation model for the $j$th variable were estimated from the set of possible auxiliary variables (the variables in $\bm{M}$ and $\bm{A}$).
            For every variable under imputation, the other variables in $\bm{T}$ were also used as predictors.
    \item MI-PCR-ALL\@.
            The PCs used in the univariate imputation model for the $j$th variable were estimated from the entire data set ($\bm{T}, \bm{M}, \bm{A}$).
            An initial single imputation step was required to obtain a complete version of $\bm{T}$ to be used exclusively to estimate the PCs.
            This step was performed by running a single chain of the mice algorithm for 20 iterations and by selecting as predictors for the imputation models all variables correlating at least $r = 0.3$ with the ones under imputation.
    \item MI-PCR-VBV\@.
            The PCs used in the univariate imputation model for the $j$th variable were estimated from all other variables ($\bm{T}_{-j}, \bm{M}, \bm{A}$), at every iteration.
\end{itemize}

We also imputed the missing data using two non-PCR methods to act as  additional points of comparison:
\begin{itemize}	
\item MI with correlation-based thresholding (MI-QP)\@.
            As a pragmatic point of comparison, this method used the \emph{quickpred} function from the R package mice \citep{mice} to select the predictors for the univariate imputaiton models via the correlation-based thresholding strategy described by \citet[pp. 687-–688]{vanBuurenEtAl:1999}.
            To implement this approach, we selected only those predictors that correlated with the imputation targets (or their associated missingness indicators) at $r = 0.1$ or higher.
            For every $j$th variable under imputation, \emph{quickpred} selected predictors from the remaining variables ($\bm{T}_{-j}, \bm{M}, \bm{A}$).
    \item MI with oracle abilities (MI-OR)\@.
            This method represented the idealized, hypothetical situation wherein the imputer knows the optimal imputation model.
	        The univariate imputation models included the other variables under imputation (which were also the analysis variables, in this case) and the predictors that were used to impose missingness ($\bm{T}_{-j}, \bm{M}$).
            For this method, we used our perfect knowledge of the missing data mechanism to define which variables should be predictors in the imputation models.
            As such, MI-OR represents an optimal point of comparison but is not replicable in practice.
\end{itemize}

To explore how the number of PCs used in MI-PCR impacts performance, we implemented the MI-PCR methods with different numbers of components.
We implemented each method with fixed numbers of components (i.e., 1, 2, $\cdots$, 10, 20, 25) as well as the maximum number of components possible (which varied by method).
In PCA, the maximum number of components cannot exceed the number of rows or columns of the data, so this number depends on the specific MI-PCR implementation:
\begin{itemize}
\item For MI-PCR-AUX, the maximum number of PCs was $56 - 4 = 52$, the number of variables in matrices $\bm{M}$ and $\bm{A}$.
\item For MI-PCR-ALL, the maximum was $56$, the total number of variables in the data set.
\item For MI-PCR-VBV, the maximum was $56 - 1 = 55$, the number of variables available as predictors for each univariate imputation model.
\end{itemize}
Using the maximum number of components addresses possible collinearity among the imputation model predictors without performing any dimensionality reduction.

Every imputation algorithm was used to obtain five imputed data sets, the default in the \emph{mice} R package.
All starting imputations were created by a simple random draw from the data.
The number of iterations was set to 20 after convergence checks\footnote{We evaluated convergence via the same procedure employed by \citet{costantiniEtAl:2022}}.

\subsubsection{Analysis and outcome measures} \label{subsubsec:analysis-and-outcome-measures}

For each data set we generated, we imputed the variables in $\bm{T}$ with the different methods described above, and we pooled the estimates of their means, variances, covariances, and correlations\footnote{We applied Fisher's $z$ transformation to the correlation coefficients before pooling.
We then back-transformed the pooled correlation coefficient estimates with the inverse Fisher's $z$ transformation \citep[p. 146]{vanBuuren:2018}.} across the multiple imputations.
The pooled estimates were stored and used to assess the performance of the imputation methods.
For a given parameter $\phi$ (e.g., mean of $\bm{x}_1$, correlation between $\bm{x}_1$ and $\bm{x}_2$), we used the absolute percent relative bias (PRB) to quantify the estimation bias introduced by the imputation procedure:
%
\begin{equation} \label{eq:prb}
\textit{PRB} = \displaystyle\left\lvert\ \frac{\bar{\hat{\phi}} - \phi}{\phi} \right\rvert \times 100
\end{equation}
%
where $\phi$ is the true value of the focal parameter defined as
$\sum_{s=1}^{S} \hat{\phi}_{s}^{full}/S$
, with
$\phi_{s}^{full}$
being the parameter estimate for the $s$th repetition computed on the original fully observed data.
The averaged focal parameter estimate under a given missing data treatment was computed as
$\bar{\hat{\phi}} = \sum_{s=1}^{S} \hat{\phi}_{s}/S$,
with
$\hat{\phi}_{s}$ being the estimate obtained from the treated incomplete data in the
$s$th data sample.
Following~\cite{muthenEtAl:1987}, we considered $\text{PRB} > 10$ as indicative of problematic
estimation bias.

To measure the statistical efficiency of the imputation methods we computed the average width of
the confidence intervals (CIW).
%
\begin{equation} \label{eq:ciw}
CIW = \frac{\sum_{s=1}^{S} \widehat{CI}^{upper}_{s} - \widehat{CI}^{lower}_{s}}{S},
\end{equation}
%
with $\widehat{CI}^{upper}_{s}$ and $\widehat{CI}^{lower}_{s}$ being the upper and lower bounds of the estimated confidence interval for the $s$-th repetition.
In general, narrower CIWs indicate higher efficiency.
However, narrower CIWs are not preferred if they come at the expense of good confidence interval coverage (CIC) of the true parameter values.
CIC is the proportion of confidence intervals that contain the true value of the parameter, across the $S$ data samples:
%
\begin{equation} \label{eq:cic}
CIC =  \frac{ \sum_{s=1}^{S} I(\phi \in \widehat{CI}_s ) }{S},
\end{equation}
%
where $\widehat{CI}_s$ is the confidence interval of the parameter estimate $\hat{\phi}_{s}$ in the $s$th replication, and $I(.)$ is the indicator function that returns 1 if the argument is true and 0 otherwise.
CIC depends on both the bias and the CIW for a parameter estimate.
An imputation method with good coverage should result in CICs greater than or equal to the nominal rate.
For 95\% CIs, CIC below 0.9 is usually considered problematic (e.g., \citealp[p. 52]{vanBuuren:2018}; \citealp[p. 340]{collinsEtAl:2001}) as it implies inflated Type I error rates.
High CIC (e.g., 0.99) implies inflated Type II error rates.

\subsection{Results}\label{subsec:results}

\subsubsection{Bias}

In Figure~\ref{fig:bias}, we report the PRB for the correlation coefficient between $\bm{x}_1$ and $\bm{x}_2$---two of the four imputed items in $\bm{T}$---in an illustrative selection of conditions.
In this report, we focus on the estimates of the correlation as this was the hardest parameter to recover (i.e., the performance differences were most pronounced) of the ones we considered.
In the supplementary material, we report the same figures for the mean, variance, and covariance.

MI-OR, MI-PCR-AUX, and MI-QP resulted in acceptable bias in all conditions (PRB $< 10$).
The bias resulting from MI-PCR-AUX depended on the number of PCs kept.
MI-PCR-AUX resulted in PRBs around or above $2.5$ when using fewer than seven PCs (i.e., the true number of latent variables), while it resulted in PRBs lower than $2.5$ using more than seven PCs.
MI-PCR-AUX with seven or more components resulted in approximately the same bias as MI-OR, outperforming MI-QP\@.
In what follows we will use the suffix -7+ to refer to any MI-PCR method using seven or more components.

MI-PCR-VBV resulted in a large bias (PRB $> 10$) when using fewer than seven PCs.
However, MI-PCR-VBV-7+ obtained PRBs lower than $10$ in all conditions.
MI-PCR-VBV-7+ produced approximately the same bias as MI-OR in all conditions, except for $nk = 2$, where it produced approximately the same PRB as MI-QP (PRB $\approx 5$).

As with the other MI-PCR methods, MI-PCR-ALL-7+ resulted in acceptable bias (PRB $< 10$).
However, while the biases of MI-PCR-AUX-7+ and MI-PCR-VBV-7+ were unaffected by the proportion of noise variables, MI-PCR-ALL-7+ produced a larger bias in the presence of a larger proportion of noise variables.
One exception to this trend was that MI-PCR-ALL-7+ always resulted in the lowest PRB of all methods when $nk = 2$.
For all other methods, bias was lowest when the possible auxiliary predictors were left in their original continuous form and was highest when the predictors were dichotomized.



\begin{figure}
\centering
\begin{knitrout}
\definecolor{shadecolor}{rgb}{0.969, 0.969, 0.969}\color{fgcolor}

{\centering \includegraphics[width=\maxwidth]{figure/plot-bias-correlation-1} 

}


\end{knitrout}
\caption{\label{fig:bias}
	Percent relative bias for the correlation between $\bm{x}_1$ and $\bm{x}_2$.
    $pn$ is the proportion of noise variables in $\bm{A}$.
    $npc$ is the number of PCs used by a given imputation method.
    The figure is organized in a grid.
    The columns of the grid refer to the different imputation methods.
    The rows differentiate the two extreme levels of the proportion of noise variables ($pn = (0, 1)$).
    The X-axis of each histogram distinguishes three discretization levels of the possible auxiliary variables ($nk = (\text{Inf}, 5, 2)$).
    For each MI-PCR method, we reported a different vertical bar for each PRB obtained using a different number of PCs ($npc = (1, \dots, 10)$).
	}
\end{figure}

\subsubsection{Confidence Intervals}

CICs for the correlation coefficient between $\bm{x}_1$ and $\bm{x}_2$ are plotted in Figure~\ref{fig:cic}.
MI-PCR-AUX-7+ and MI-PCR-VBV-7+ resulted in the lowest deviations from nominal coverage (CIC $\approx 0.95$), while MI-QP always resulted in under-coverage of the true parameter values (CIC $< 0.90$).
Only MI-PCR-VBV-7+ tended towards over-coverage of the true parameter values (CIC $> 0.95$).
However, MI-PCR-VBV-7+ did produce under-coverage when $nk = 2$, resulting in CIC $\approx 0.75$, the same as MI-QP\@.
Finally, MI-PCR-ALL showed more severe under-coverage than the other MI-PCR methods in all conditions except $nk = 2$.



\begin{figure}
\centering
\begin{knitrout}
\definecolor{shadecolor}{rgb}{0.969, 0.969, 0.969}\color{fgcolor}

{\centering \includegraphics[width=\maxwidth]{figure/plot-cic-correlation-1} 

}


\end{knitrout}
\caption{\label{fig:cic}
	Confidence interval coverage for the correlation between $\bm{x}_1$ and $\bm{x}_2$.
    $pn$ is the proportion of noise variables in $\bm{A}$.
    $npc$ is the number of PCs used by a given imputation method.
    The figure is organized in a grid.
    The columns of the grid refer to the different imputation methods.
    The rows differentiate the two extreme levels of the proportion of noise variables ($pn = (0, 1)$).
    The X-axis of each histogram distinguishes three discretization levels of the possible auxiliary variables ($nk = (\text{Inf}, 5, 2)$).
    For each MI-PCR method, we reported a different vertical bar for each CIC obtained using a different number of PCs ($npc = (1, \dots, 10)$).
	}
\end{figure}

Figure 3 shows the average CIW for the correlation between $\bm{x}_1$ and $\bm{x}_2$.
All MI-PCR methods using at least seven components produced narrower confidence intervals than the intervals obtained with MI-QP\@.
When using more than seven components, MI-PCR-ALL resulted in the narrowest confidence intervals, followed by MI-PCR-VBV, and MI-PCR-AUX\@.
However, the confidence intervals obtained with MI-PCR-ALL and MI-PCR-VBV almost doubled in size when using fewer than seven components.
MI-PCR-AUX was less influenced by the number of PCs, providing only slightly wider confidence intervals when using fewer than seven components.
Finally, MI-PCR-VBV-7+ and MI-PCR-AUX-7+ resulted in essentially the same CIW when the auxiliary variables were binary.



\begin{figure}
\centering
\begin{knitrout}
\definecolor{shadecolor}{rgb}{0.969, 0.969, 0.969}\color{fgcolor}

{\centering \includegraphics[width=\maxwidth]{figure/plot-ciw-correlation-1} 

}


\end{knitrout}
\caption{\label{fig:ciw}
	Average confidence interval width for the correlation between $\bm{x}_1$ and $\bm{x}_2$.
    $nk$ is the number of categories for the items in matrices $\bm{M}$ and $\bm{A}$.
    $pn$ is the proportion of noise variables in $\bm{A}$.
	}
\end{figure}

\subsection{Discussion}

The most important factor influencing the performance of the MI-PCR methods was the number of components used.
This result followed a very clear, dichotomous pattern: using fewer than seven components led to poor performance across all outcome measures for all MI-PCA methods, whereas using more than seven components universally produced much better performance.
As we generated the data based on seven latent variables, this result suggests that researchers using MI-PCR must employ at least as many components as there are latent variables in the data generating model.
Thankfully, our results suggest no substantial consequences for using more components than necessary.

For all methods except MI-PCR-ALL, bias was higher when the potential auxiliary variables were discretized to fewer categories.
This pattern probably reflects the loss of observed information caused by discretization.
As a result of discretization, the association between variables is attenuated, which makes every auxiliary predictor less useful as an imputation model predictor.
Furthermore, missing values were imposed on the target variables based on the continuous variables in set $\bm{M}$.
When the variables in set $\bm{M}$ were discretized, they became poorer representations of the actual MAR predictors.
As a result, even MI-OR follows a trend of increasing bias for decreasing numbers of categories.
The discretization of the possible auxiliary variables did not seem to impact the performance of MI-PCR more than it impacted other approaches.

For the most part, the proportion of noise variables in the set of possible auxiliary variables did not have a strong impact on the performance of the MI-PCR methods.
In the simulation study, a higher proportion of noisy variables resulted in higher bias when fewer than seven components were selected.
However, when enough PCs were kept, the MI-PCR methods' performances were indistinguishable across different proportions of noisy variables.

As for the different ways of using PCA within MICE, the variable-by-variable approach seems to be the most promising.
Although sometimes outperformed by MI-PCR-AUX (e.g., when using fewer than seven components or when the potential auxiliary variables were dichotomized), MI-PCR-VBV produced low bias, good coverage, and its competitive imputation performance was also accompanied by a few other desirable features.
Compared to the other MI-PCR approaches, when MI-PCR-VBV deviated from nominal coverage, it showed a tendency toward over-coverage.
An imputation method characterized by over-coverage will inflate type II error rates, making inferences more conservative than they should be.
Although this is undesirable, it is usually less worrisome than the problem of under-coverage, which makes the rejection of the null hypothesis more likely than it should be.
Furthermore, MI-PCR-VBV does not rely on a previous single imputation step to obtain complete-data for extracting PCs.
By performing PCA at every iteration, there is no need to pre-impute the variables from which PCs are extracted.
Finally, MI-PCR-VBV does not require knowledge of the analysis model, while MI-PCR-AUX needs this knowledge to distinguish which variables in the data should be summarized by PCs and which variables should be used in their raw form.
At the same time, MI-PCR-VBV can still incorporate important features of the analysis model, if these features are known before imputation.
Analysis model variables can be included in any desired functional form as predictors in the imputation models and excluded from the PC estimation.
In such a scenario, MI-PCR-VBV would supplement each imputation model with PCs representing information that would have otherwise been ignored by the imputation procedure.


==> section_04.tex <==
% Project:  paper-mipcr-compare
% Topic:    Present fireworks disaster data comparison
% Author:   Edoardo Costantini
% Created:  2021-12-20
% Modified: 2022-06-09

\section{Case study: fireworks disaster data}\label{sec:case-study}

To understand the performance of MI-PCR on real data, we compared the performance of MI-PCR with an imputation procedure carried out by an imputation expert on a real-world data set.
\citet[pp. 315--317]{vanBuuren:2018} gives a detailed description of how he solved the ``many variables'' problem for the Fireworks' disaster data set (FDD).
On May 13, 2000, the explosion of a fireworks storage facility in Enschede, the Netherlands, killed 23 people and injured about 950.
Many people residing in the neighborhood of the explosion experienced signs of post-traumatic stress disorder (PTSD).
The FDD was collected as part of a randomized controlled trial carried out in the aftermath of the explosion.
The data were collected to assess the efficacy of two treatments of anxiety-related disorders in children, in terms of reducing PTSD symptoms over time.
The main outcome measure for this analysis was the PTSD Reaction Index (PTSD-RI), measured as reported by the child and by the parent, at three different time points.
Fifty-two children were assigned either Eye Movement Desensitisation and Reprocessing (EMDR) treatment, or Cognitive Behavioral Therapy (CBT).
Of the 65 variables recorded in the data set, 49 were incomplete.
The percentage of missing values on each variable ranged from 3\% to 50\%.
A complete-case analysis would have resulted in analyzing only eight cases.
To avoid the unacceptable reduction in sample size and the risk of biased estimates, a different missing data treatment was needed.

The major difficulty in imputing these data was the large number of predictors relative to the sample size ($p > n$).
To avoid over-parametrized imputation models, the imputation models' predictors needed to be carefully selected.
Van Buuren employed two main strategies to address the high-dimensional nature of the data:
\begin{itemize}
    \item Use only the first measurement of the outcomes as predictors in the imputation models of other outcomes.
        This choice reduced the number of predictors by two-thirds.
    \item Use the total scores of scales as predictors in the univariate imputation models of other variables, instead of the individual scale items.
            This was done using passive imputation (\citealp[p. 12]{vanBuurenOudshoorn:2000}; \citealp[pp. 1129--1130]{eekhoutEtAl:2018}).
\end{itemize}

Each of the three MI-PCR strategies considered in this report is suitable to address the large number of possible imputation model predictors in the FDD\@.
The advantage of MI-PCR is the automatic way in which large numbers of predictors can be accommodated.
Through this case study, we wish to illustrate the degree to which MI-PCR can produce results similar to those obtained by an expertly designed imputation procedure.
There are several reasons why the FDD is ideally suited to these purposes:
\begin{itemize}
    \item The data have key characteristics of social and behavioral science data sets (e.g., composite scales, longitudinal data).
    \item The code Van Buuren used to perform the MI procedure is freely accessible.
    \footnote{\url{https://github.com/stefvanbuuren/fimdbook/blob/master/R/fimd.R}}
    \item The data are freely accessible through the \emph{mice} R package~\citep{mice}.
    \item The reasoning behind the expert's MI procedure is well documented~\citep[p. 313]{vanBuuren:2018}.
\end{itemize}

\subsection{Method}\label{subsubsec:case-method}
The main analysis reported in \citet[p. 313]{vanBuuren:2018} focused on the effect of treatment on the mean PTSD-RI scores (both child-reported and parent-reported) across three time points.
Therefore, six variables were analyzed: the PTSD-RI total scores reported by children and their parents at three different time points.
We imputed these six analysis variables with the three MI-PCR procedures evaluated above and compared the pooled means obtained thereby with the results of Van Buuren's imputation procedure.
To evaluate the variability of the imputation methods, we repeated this procedure with 20 different random number seeds.

The results of the simulation study suggested that MI-PCR performs poorly if an insufficient number of components is extracted, whereas its performance is not severely impacted by selecting too many components.
Therefore, to choose the number of PCs in this case study, we decided to use the maximum number of PCs allowed by each imputation procedure.
The two variables with the most missing values had 25 cases observed.
Hence, at most 24 predictors could be used for each imputation model, and we could use at most 24 PCs.

We specified MI-PCR-AUX to impute the six items under analysis.
In each of the six univariate imputation models, MI-PCR-AUX used as predictors the other five variables under imputation and the first 19 PCs estimated from the remaining auxiliary columns (5 + 19 = 24).
We performed single imputation on the potential auxiliary variables to allow the PC estimation.
We used predictive mean matching as univariate imputation method and kept the imputations obtained after 20 iterations.
The predictors for the imputation models were selected by correlation-thresholding, with the threshold set to $0.1$.

The MI-PCR-ALL method used the first 24 PCs estimated on the entire data set---including the 6 analysis variables---as the sole predictors in each of the six univariate imputation models.
The same single imputation specification used for MI-PCR-AUX was used here to generate the complete data on which to estimate PCA\@.
Finally, MI-PCR-VBV was performed by extracting 24 components from all the variables not under imputation for each univariate imputation model, at every iteration of the mice algorithm.
All starting imputations were created by a simple random draw from the data.

\subsection{Results}\label{subsubsec:case-results}
Figures~\ref{fig:fdd-yp} and~\ref{fig:fdd-yc} report the (pooled) mean level of PTSD-RI over the three time points after imputation with the following approaches:
\begin{itemize}
    \item Expert's imputation models;
    \item The three MI-PCR approaches;
    \item Default run of \emph{mice} without any pre-processing and using all default argument values.
\end{itemize}

While all methods led to similar trends, variability of the imputations was noticeably higher for MI-PCR-AUX, MI-PCR-ALL, and the default run of \emph{mice}.
At every time point, the 20 different pooled means of the analyzed variables spread over a wider range of values compared to the expert's imputation.
This pattern held for both outcome variables, but it was most conspicuous for the child-reported PTSD-RI\@.
MI-PCR-AUX and MI-PCR-ALL had lower imputation precision than even the default run of \emph{mice} in this setup.
The performance of MI-PCR-VBV was on par with that of the expert's imputation: both methods produced comparable location and spread of the outcome variables pooled means.



\begin{figure}
\centering
\begin{knitrout}
\definecolor{shadecolor}{rgb}{0.969, 0.969, 0.969}\color{fgcolor}

{\centering \includegraphics[width=\maxwidth]{figure/plot-fdd-yp-1} 

}


\end{knitrout}
\caption{\label{fig:fdd-yp}
	Mean levels of PTSD-RI parent score after imputation.
    The multiple lines plotted for each method represent results obtained with 20
    different seeds.
	}
\end{figure}



\begin{figure}
\centering
\begin{knitrout}
\definecolor{shadecolor}{rgb}{0.969, 0.969, 0.969}\color{fgcolor}

{\centering \includegraphics[width=\maxwidth]{figure/plot-fdd-yc-1} 

}


\end{knitrout}
\caption{\label{fig:fdd-yc}
	Mean levels of PTSD-RI children score after imputation.
    The multiple lines plotted for each method represent results obtained with 20
    different seeds.
	}
\end{figure}


==> section_05.tex <==
% Project:  paper-mipcr-compare
% Topic:    Conclusions
% Author:   Edoardo Costantini
% Created:  2021-12-17
% Modified: 2022-06-08

\section{Conclusions}\label{sec:conclusions}

Dimensionality reduction through PCA can be an effective and automatic way to address many possible predictors during missing data imputation.
In our simulation study, using PCR as a univariate imputation method within every iteration of a MICE algorithm (i.e., MI-PCA-VBV) provided small bias, good statistical efficiency, and close to nominal coverage.
So long as the number of PCs met or exceeded the true number of latent variables, MI-PCR-VBV outperformed the standard correlation-thresholding approach (MI-QP) on all the metrics we considered.
Furthermore, the good imputation performance of MI-PCR-VBV comes with some desirable features that are missing from the other MI-PCR methods.
First, MI-PCA-VBV does not rely on knowledge of the analysis model, although such knowledge is easily incorporated when available.
Second, MI-PCA-VBV does not require a pre-processing single imputation step.
Third, when MI-PCR-VBV resulted in deviations from nominal coverage, it tended towards over-coverage.
Finally, in the case study, MI-PCR-VBV was able to automatically obtain results that were essentially indistinguishable from those produced by an expertly designed imputation model.


==> section_06.tex <==
% Project:  paper-mipcr-compare
% Topic:    Limitations and future directions
% Author:   Edoardo Costantini
% Created:  2021-12-17
% Modified: 2022-06-08

\section{Limitations and future directions}\label{sec:limitations}

The study we report here provides compelling evidence for the strong performance of MI-PCA methods, but these results must be considered in light of certain limitations.
We selected the number of variables in the simulation study (56) to be large enough to require a careful set-up of the imputation models, but this value is still somewhat small relative to most common social science data sets.
To maintain reasonable simulation run times, we decided to generate data sets with tens of variables instead of hundreds, though the latter may be more realistic.
We have no reason to believe that this decision has materially affected our findings, but it is possible that larger data sets or more incomplete variables could affect the performance of the methods we evaluate here.

When specifying imputation models, the predictors included in the model should explain as much variance as possible in the target variables.
However, the MI-PCR implementations we compared here extract PCs without considering the relationship between the variables going into the PCs and the variables under imputation.
In other words, the MI-PCR methods we evaluated could extract components that explain relatively little variance in the variables under imputation.
To address this possibility, MI-PCR-VBV could potentially be improved by incorporating some form of supervision, such as supervised PCA \citep{bairEtAl:2006} or principal covariates regression \citep{deJongKiers:1992}.

The uniquely good performance of MI-PCR-ALL in the conditions with dichotomized auxiliary variables remains something of a mystery.
We did not expect this pattern, and we do not have a good explanation for this finding.
Since the other MI-PCR methods performed at their worst in the $nk = 2$ condition, it would be interesting to further explore the capabilities of MI-PCR-ALL in this special case.

Finally, multilevel data provide another interesting avenue for future research.
Social science data are often characterized by clusters of observations.
Imputation procedures that ignore this feature of the data can lead to biased estimates as imputations are generated without considering cluster dependencies~\citep{reiterEtAl:2006}.
One way to address this issue is to include dummy variables representing the cluster effects in the imputation models~\citep[fixed effect imputation,][]{enders:2016}.
However, this approach has the disadvantage of increasing the dimensionality of the design matrix to an impractical extent.
Using PCs to reduce dimensionality might be a good way to address grouping in the data without incurring estimation difficulties of sophisticated multilevel imputation procedures.


==> section_abstract.tex <==
% Project:  paper-mipcr-compare
% Topic:    Abstract
% Author:   Edoardo Costantini
% Created:  2021-12-17
% Modified: 2022-06-09

Multiple Imputation (MI) is one of the most popular approaches to addressing missing values in questionnaires and surveys.
MI with multivariate imputation by chained equations (MICE) allows flexible imputation of many types of data.
In MICE, for each variable under imputation, the imputer needs to specify which variables should act as predictors in the imputation model.
The selection of these predictors is a difficult, but fundamental, step in the MI procedure, especially when there are many variables in a data set.
In this project, we explore the use of principal component regression (PCR) as a univariate imputation method in the MICE algorithm to automatically address the ``many variables'' problem that arises when imputing large social science data.
We compare different implementations of PCR-based MICE with a correlation-thresholding strategy through two Monte Carlo simulation studies and a case study.
We find the use of PCR on a variable-by-variable basis to perform best and that it can perform closely to expertly designed imputation procedures.


==> section_biblio.tex <==
% Project:  paper-mipcr-compare
% Topic:    Bibliography
% Author:   Edoardo Costantini
% Created:  2021-12-17
% Modified: 2021-12-17

\bibliographystyle{./style/asj}

\bibliography{
	\pathBIB/missingData/bibtex/papers,
	\pathBIB/missingData/bibtex/books,
	\pathBIB/missingData/bibtex/software,
	\pathBIB/bayesStats/bibtex/papers,
	\pathBIB/programming/bibtex/papers,
	\pathBIB/survey/bibtex/data,
	\pathBIB/survey/bibtex/studies,
	\pathBIB/statsLearn/bibtex/books,
	\pathBIB/statsLearn/bibtex/papers,
	\pathBIB/statsLearn/bibtex/software
	}

==> section_conflict.tex <==
% Project:  paper-mipcr-compare
% Topic:    Conflict of interest
% Author:   Edoardo Costantini
% Created:  2021-12-17
% Modified: 2021-12-17

No authors reported any financial or other conflicts
of interest in relation to the work described.

==> section_funding.tex <==
% Project:  paper-mipcr-compare
% Topic:    Funding information
% Author:   Edoardo Costantini
% Created:  2021-12-17
% Modified: 2022-05-27

Not applicable
